Dynamics Transfer GAN: Generating Video by Transferring Arbitrary Temporal Dynamics from a Source Video to a Single Target Image

In this paper, we propose Dynamics Transfer GAN; a new method for generating video sequences based on generative adversarial learning. The spatial constructs of a generated video sequence are acquired from the target image. The dynamics of the generated video sequence are imported from a source video sequence, with arbitrary motion, and imposed onto the target image. To preserve the spatial construct of the target image, the appearance of the source video sequence is suppressed and only the dynamics are obtained before being imposed onto the target image. That is achieved using the proposed appearance suppressed dynamics feature. Moreover, the spatial and temporal consistencies of the generated video sequence are verified via two discriminator networks. One discriminator validates the fidelity of the generated frames appearance, while the other validates the dynamic consistency of the generated video sequence. Experiments have been conducted to verify the quality of the video sequences generated by the proposed method. The results verified that Dynamics Transfer GAN successfully transferred arbitrary dynamics of the source video sequence onto a target image when generating the output video sequence. The experimental results also showed that Dynamics Transfer GAN maintained the spatial constructs (appearance) of the target image while generating spatially and temporally consistent video sequences.

==> sections/03-method-3-Training-old.tex <==
The training of the Dynamics Transfer GAN is a 2-player zero-sum game problem. Specifically, in this paper, the generative part of the network is a group of networks, i.e., the dynamics channel embedder $(F)$ and the generator network $(G)$. The discriminative part of Dynamics Transfer GAN is both the spatial discriminator $(D_s)$ and the dynamics discriminator $(D_d)$ networks. Note that the RNN parameters in the appearance suppressed dynamics feature encoder $(A)$ are frozen. Thus, they are not included in the gradient update process. Explicitly, the training of $F, G, D_s$, and $D_d$ is achieved by solving the minimax problem with the value function:
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
&\underset{F,G}{\min}\,\underset{D_s,D_d}{\max} \, \mathcal{L}(F,G,D_s,D_d) = 
\mathbb{E}_{\textbf{y} \sim p_{\textbf{y}} }[\log{(D_s(\textup{\textbf{Y})}}] \nonumber\\
&+ \mathbb{E}_{\textbf{z}^{(d)} \sim p_{\textbf{z}}^{(d)} }[\log{(D_d(\textbf{z}}_{\textup{T}}^{(d)}))]  \nonumber\\
&+ \mathbb{E}_{\textbf{Z}^{(d)} \sim p_{\textbf{Z}}^{(d)},\textbf{Z}^{(s)} \sim p_{\textup{\textbf{Z}}}^{(s)} }[\log{(1-D_s(G(\textup{\textbf{Z}}}^{(s)},F(\textup{\textbf{Z}}^{(d)}))))]  \nonumber\\ 
&+ \mathbb{E}_{\widehat{\textbf{z}}^{(d)} \sim p_{\textbf{z}}^{(d)} }[\log{(1-D_d(\widehat{\textbf{z}}}_{\textup{T}}^{(d)}))].
\end{align}
\label{eq:2}
%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}
       
Note that the back propagation can be performed independently on the discriminator networks $(D_d, D_s)$. The generative networks $(F, G)$ are updated after both discriminators $(D_d, D_s)$. Therefore, in practice, the training of the discriminators $(D_d, D_s)$ and that of the generative networks $(F, G)$ are performed alternatively. In the first step, discriminators $(D_d, D_s)$ are trained as:
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
&\underset{D_s}{\max} \, \mathcal{L}_{D_s}(F,G,D_s) = \mathbb{E}_{\textbf{y} \sim p_{\textbf{y}} }[\log{(D_s(\textup{\textbf{Y})}}] \nonumber\\
&+ \mathbb{E}_{\textbf{Z}^{(d)} \sim {p_{\textbf{Z}^{(d)}}}, \textbf{Z}^{(s)} \sim {p_{\textbf{Z}^{(s)}}} }[\log{(1-D_s(G(\textup{\textbf{Z}}}^{(s)},F(\textup{\textbf{Z}}^{(d)}))))]  \nonumber\\ 
&\underset{D_d}{\max} \, \mathcal{L}_{D_d}(F,G,D_d) = \mathbb{E}_{\textbf{z}^{(d)} \sim p_{\textbf{z}^{(d)}} }[\log{(D_d(\textbf{z}}_{\textup{T}}^{(d)}))]  \nonumber\\
&+ \mathbb{E}_{\widehat{\textbf{z}}^{(d)} \sim {p_{\textbf{z}^{(d)}}} }[\log{(1-D_d(\widehat{\textbf{z}}}_{\textup{T}}^{(d)}))].
\end{align}
\label{eq:3}
%%%%%%%%%%%%%%%%%%%%
In the second step, the generative parts of the network are trained as: 
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
\underset{F,G}{\min}\, \mathcal{L}(F,G,D_s,D_d) = -[\mathbb{E}_{\widehat{\textbf{z}}^{(d)} \sim p_{\textbf{z}^{(d)}} }[\log{(D_d(\widehat{\textbf{z}}}^{(d)}))] \nonumber\\
 - \mathbb{E}_{\textbf{Z}^{(d)} \sim p_{\textbf{Z}^{(d)}},\textbf{Z}^{(s)} \sim p_{\textbf{Z}^{(s)}} }[\log{(D_s(G(\textup{\textbf{Z}}}^{(s)},F(\textup{\textbf{Z}}^{(d)}))))].
\end{align}
\label{eq:4}
%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}

Adding a reconstruction term to the generative networks could improve the quality of the generated images \cite{7}, We employ L1 frame reconstruction loss to improve the spatial reconstruction at each frame as follows:
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_{G^{(s)}}(F,G) = \mathbb{E}_{\textbf{y} \sim p_{\textbf{y}}} [\left \| \textbf{y}- G(\textbf{z}^{(s)}, F(\textbf{z}^{(d)})) \right \|].  
\end{align}
\label{eq:5}
%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}

Finally, to maintain dynamic consistency even when the sequence is lengthy, we propose a reconstruction term on the appearance suppressed dynamics feature. Unlike the loss from the dynamics discriminator (which is calculated at the end of the sequence), this term makes sure that the generated sequence dynamics are maintained at each frame. 
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
\mathcal{L}_{G^{(d)}}(F,G) = \mathbb{E}_{\textup{\textbf{Z}}^{(d)} \sim p_{\textup{\textbf{Z}}^{(d)}}} [\left \| \textup{\textbf{Z}}^{(d)}- \widehat{\textup{\textbf{Z}}}^{(d)} \right \|].  
\end{align}
\label{eq:6}
%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5cm}

By plugging in eqs. (5) and (6) in the second step of the training described in eq.(4), the generator training can be obtained by calculating the loss:
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%
\begin{align}
&F^*, G^* = - \underset{F,G}{\min}\, [\lambda_{DGAN} \mathcal{L}(F,G,D_s,D_d) \nonumber\\
&+ \lambda_{G^{(s)}} \mathcal{L}_{G^{(s)}}(F,G)
+ \lambda_{G^{(d)}} \mathcal{L}_{G^{(d)}}(F,G)],
\end{align}
\label{eq:7}
%%%%%%%%%%%%%%%%%%%%
where $\lambda_{DGAN}$, $\lambda_{G^{(s)}}$, and $\lambda_{G^{(d)}}$  are hyper-parameters to control the generative loss term. $\lambda_{DGAN}$ is the weight controlling the generative loss of the Dynamics Transfer GAN described in eq. (4), $\lambda_{G^{(s)}}$ is the weight controlling the frame reconstruction loss detailed in eq. (5), and $\lambda_{G^{(d)}}$ is the weight controlling the loss that maintains the dynamic consistency at each frame described in eq. (6).


==> sections/04-experiments-1-Implementation.tex <==
The training and implementation of the proposed Dynamics Transfer GAN have been conducted using TensorFlow \cite{29}. The dynamic channel embedder $(F)$, and the dynamics discriminator $(D_d)$ were constructed of a stack of fully connected layers. The encoder part of the generator network $(G)$ was constructed of a stack of convolutions that followed the structures: 2D convolution, batch normalization \cite{30} and lrelu \cite{31}. The first convolutional layer (Conv1) of the encoder part was an exception. Conv1 did not contain a batch normalization stage. For the decoder part of $G$, deconvolution layers were utilized that followed the structure: fractionally strided convolutional \cite{32}, batch normalization, and relu \cite{33}. The relu at activation at the last deconvolution layer was replaced with a hyper tangent activation. Similar to the decoder part of $G$, the spatial discriminator network $(D_s)$ was constructed of 5 convolution layers. The First four of which followed the structure: 2D convolution, batch normalization, and lrelu activation. The fifth layer was constructed by a 2D convolution followed by a sigmoid activation. The structure of Dynamics transfer GAN is detailed in the supplementary material.
